On the Parameter Identifiability of Partially Observed Linear Causal Models

Linear causal models are important tools for modeling causal dependencies and yet in practice, only a subset of the variables can be observed. In this paper, we examine the parameter identifiability of these models by investigating whether the edge coefficients can be recovered given the causal structure and partially observed data. Our setting is more general than that of prior research - we allow all variables, including both observed and latent ones, to be flexibly related, and we consider the coefficients of all edges, whereas most existing works focus only on the edges between observed variables. Theoretically, we identify three types of indeterminacy for the parameters in partially observed linear causal models. We then provide graphical conditions that are sufficient for all parameters to be identifiable and show that some of them are provably necessary. Methodologically, we propose a novel likelihood-based parameter estimation method that addresses the variance indeterminacy of latent variables in a specific way and can asymptotically recover the underlying parameters up to trivial indeterminacy. Empirical studies on both synthetic and real-world datasets validate our identifiability theory and the effectiveness of the proposed method in the finite-sample regime. Code: https://github.com/dongxinshuai/scm-identify.

==> 13-draft.tex <==
\section{After NeurIPS Submission}
\begin{flalign*}
\Sigma_{X}
& =(I-D)^{-T}\Big(\Omega_\set{X}+B^{T} M^{T} \Omega_\set{L} M B+\Omega_\set{X}(I-D)^{-1} C M B+B^{T} M^{T} C^{T}(I-D)^{-T} \Omega_\set{X} \\
& \qquad\qquad\qquad\qquad +B^{T} M^{T} C^{T}(I-D)^{-T} \Omega_\set{X}(I-D)^{-1} C M B\Big)(I-D)^{-1}\\
&=(I-D)^{-T}\Big(B^{T} M^{T} \Omega_\set{L} M B+(I+NB)^T\Omega_X(I+NB)\Big)(I-D)^{-1}
\end{flalign*}

==> deprecated.tex <==
% Causal Representation Learning (CRL) aims to construct compact representations that capture the data generation processes from observed data. In temporal contexts, CRL achieves this by inverting the mixing function that transforms hidden factors into observations and by identifying the transitions that govern the underlying hidden causal dynamics. However, when the transitions are nonstationary which are characterized by multiple distribution shifts across different domains, the task of learning causal representations becomes particularly challenging, especially when the domains or distribution shifts are unobserved. This limitation significantly restricts the applicability of CRL in real-world sequential processing systems. To overcome these limitations and bridge the theoretical-practical gap, we leverage sparse transition assumption which aligned with human intuition and present the identifiability result from a theoretical perspective and then introduce a novel framework: \emph{\fullmethodname}~(\method) to reliably identify both distribution shifts and hidden factors. The results of the experiment on both synthetic and real-world datasets demonstrate a significant improvement over existing baselines.
    
    % Causal Representation Learning (CRL) has attracted increasing attention from both the causality and machine learning communities.
    % In the analysis of temporal or sequential data, recent research has exploited the sparsity or variability of transitions in temporal causal dynamics to enhance identifiability, provided that some forms of \emph{observed} interventions or distribution shifts are available.
    % However, such conditions are often challenging to meet in real-world scenarios without extensive human annotation and crowd-sourced labeling.
    % To bridge the gap between theoretical advances and practical applications, we propose a method that reliably recovers both distribution shifts and latent factors in temporal causal dynamics under sparsity constraints, even when these domain shifts are unknown and unobserved, as long as the changes across different domains are significant.
    % Our approach, \textbf{N}onstationary \textbf{S}parse \textbf{C}ausal \textbf{T}emporal \textbf{R}epresentation \textbf{L}earning~(\method), utilizes a VAE-based framework where domain variables and latent causal dynamics are efficiently learned and regularized through sparsity constraints.
    % Experiments conducted on both synthetic and real-world datasets validate the effectiveness of NSCTRL by demonstrating a quite significant margin above baselines.



% Causal reasoning for sequence data is a long-lasting yet fundamental task~\cite{berzuini2012causality,ghysels2016testing,friston2009causal}.
% The majority of the studies focus on the temporal causal discovery among observed variables~\cite{granger1980testing,gong2015discovering,hyvarinen2010estimation}.
% However, in many real-world scenarios, the observed data (e.g., image pixels in videos) instead of having direct causal edges, are generated by some causally related latent temporal processes or confounders.
% Learning causal relations has practical use cases, which benefit a lot of downstream tasks.
% However, estimating latent causal structures among those unobserved variables purely from observations without appropriate class of assumptions is an extremely challenging task~\cite{locatello2019challenging,hyvarinen1999nonlinear}.

% Under the topic of unsupervised representation learning via nonlinear Independent Component Analysis (ICA), some strong identifiability results of the latent variables have been established~\cite{hyvarinen2016unsupervised,hyvarinen2017nonlinear,hyvarinen2019nonlinear,khemakhem2020variational,sorrenson2020disentanglement,halva2020hidden} by introducing side information such as class labels and domain indices. 
% Specifically focusing on time-series data, history information is also widely used as the side information for the identifiability of latent processes~\cite{halva2021disentangling,klindt2020towards,yao2021learning,yao2022temporally}. 
% However, existing studies mainly focused on and derived identifiability results in stationary settings~\cite{hyvarinen2017nonlinear,klindt2020towards}, in which the temporal transitions are fixed over time, or nonstationary settings with explicitly observed domain indices~\cite{khemakhem2020variational,yao2021learning,yao2022temporally}.

% One can immediately tell the infeasibility of those two scenarios because the general time series data are usually nonstationary and the nonstationary information~(class labels and domain indices) is usually hard to acquire.
% That is particularly true when considering real-world data, such as video or signal sequences. It does not make sense to assume that there exists a stationary transition function that is applied to the whole video clip. Instead of using a rather complex transition function to describe the whole video clip, a more reasonable approach is that the whole sequence can be divided into multiple atomic segments and the same transition function is shared within the same segment, but across different segments, the transition functions are different; in other words, the transition function can be expressed as a function of the domain index. Also, it is worth mentioning that if such domain or regime indices are latent or unobserved, then we cannot directly utilize the existing framework to learn the latent causal dynamics. That is again a more realistic case that in general, the domain indices within a video are not accessible without expensive human annotation.

% Recently, HMNLICA~\cite{halva2020hidden}, NCTRL~\cite{song2023temporally}, and attempted to resolve the problem by introducing Markov Assumption on the nonstationary discrete domain variable, they assumed the domain indices follow a first-order Markov Chain and estimated the domain information purely from observed data. However, HMNLICA assumes temporally mutually independent sources in the data-generating process (conditioning on domain indices), i.e. they don't allow latent factors to have time-delayed causal relations in between. Such an assumption imposed a huge negative impact on the usability of those methods. NCTRL To accommodate for such general sequential data, time-delayed temporal dependence should be considered in the latent $\mathbf{z}_t$ space (Fig \ref{fig:pgm-d}, otherwise, it is impossible to model a complex video data's temporal relation purely from discrete, domain indices. Also to make sure that the latent independent components can be recovered, temporally conditional independence should also be enforced, i.e. Each dimension of $\mathbf{z}_t$ is conditionally independent given the history $\mathbf{z}_{\text{history}}$. To this end, a natural question is:
% \begin{center}
% 	{\bf \textit{How can we establish identifiability of nonlinear ICA for general sequential data with nonstationary causally-related process without observing auxiliary variable?}}\\
%         % {\bf \textit{nonstationary causally-related process without observing auxiliary variable?} } 
%  % \\{\bf \textit{} }
% \end{center}
% formulate question 
% To answer this question, we first formulate the latent nonstationary states as a discrete Markov process and further explore the Markov Assumption~\cite{gassiat2016inference} which is introduced for identifiability of nonlinear ICA in HMNLICA~\cite{halva2020hidden} and use stronger identifiability result corresponding to the conditional emission distribution~(i.e. the transition function of different domains) and the transition matrix of the Markov process. Specifically, we leverage the identifiability of Autoregressive Hidden Markov Models in \cite{balsells-rodas2023on} to accommodate time-delayed causally-related non-parametric transitions in latent space. Then we utilize the linear independence (Thm. \ref{thm2: identifiability of z}) to further establish the identifiability of $\mathbf{z}_t$.

% The main contributions of this work can be summarized as follows:
% \begin{itemize}
%     \item To our best knowledge, this is the first identifiability result that can handle the nonstationary time-delayed causally-related latent temporal processes without the auxiliary variable. We formulate the problem, especially the nonstationary states into the Markov process, establish identifiability purely from observed data, and then show strong identifiability of latent independent components.
%     \item We present \method, \textbf{N}onstationary \textbf{S}parse \textbf{C}ausal \textbf{T}emporal \textbf{R}epresentation \textbf{L}earning a VAE-based method in which the latent causal dynamics is efficiently learned and regularized via sparsity constraints.
%     \item Experiments on both synthetic and real-world datasets demonstrate the effectiveness of the proposed method in recovering the latent variables.
% \end{itemize}
% To handle this, dividing the sequence into segments, each sharing a transition function internally but varying between segments, effectively making the transition function dependent on the domain index. Moreover, if domain indices are unobserved, existing frameworks cannot be directly applied to learn latent causal dynamics, which represents a more realistic scenario where domain indices are unobservable without extensive human annotation.

% Recent approaches \cite{halva2020hidden, balsells2023identifiability, song2023temporally} have attempted to overcome these challenges by adopting a Markovian structure for nonstationary domain variables and deducing domain indices directly from observed data. However, these methods face notable constraints; they struggle with modeling time-delayed causal relationships in latent spaces, and the Markov property is insufficient for effectively capturing the arbitrary nonstationary variations in domain variables. This leads us to the following question.
